An Exponential Sample-Complexity Advantage for Coherent Quantum Inference

Standard quantum inference converts quantum data into classical outputs. We study an alternative inference setting in which the desired output is quantum. Such settings include quantum purity amplification (QPA), random purification and approximate cloning, and density matrix exponentiation. We show that such protocols can achieve exponentially lower sample complexity than incoherent, measurement-mediated protocols, establishing, to the best of our knowledge, the first nontrivial separations between dimension-independent coherent and dimension-dependent incoherent sample complexity. For QPA with principal-eigenstate targets and $d$-dimensional inputs, at fixed output number and spectral gap, coherent processing achieves error $\varepsilon$ using $O(1/\varepsilon)$ copies, whereas any incoherent protocol requires $\Omega(d/\varepsilon)$ copies. Together, these separations motivate a unified picture of coherent quantum inference, in which an entanglement-breaking limit identifies the optimal incoherent counterpart.

==> ci_notation.tex <==
\begin{table}[htbp]
\centering
\caption{Summary of key mathematical notations used in the paper and the Supplemental Material.}
\label{tab:mathematical_notation}
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{\textwidth}{@{}l X l@{}}
\toprule
\textbf{Symbol} & \textbf{Description} & \textbf{Main Usage / Definition} \\
\midrule
$\mathcal{X}$ & Input state space (set of density operators on the input Hilbert space). & \cref{def:cqi_protocol} \\
$\Gamma(\Sigma)$ & Target quantum state mapping (the ideal output state). & \cref{def:cqi_protocol} \\
$\mathcal{T}$ & Coherent quantum inference (CQI) protocol (quantum channel). & \cref{def:cqi_protocol} \\
$L(\Gamma(\Sigma), \Sigma')$ & Loss function quantifying performance of protocol output $\Sigma'$ relative to $\Gamma(\Sigma)$. & \cref{def:cqi_protocol} \\
$\mathcal{L}_{\mathrm{m}}$, $\mathcal{L}_{\mathrm{b}}$ & Minimax risk (worst-case loss) and Bayesian risk (average loss under prior $\pi$). & \cref{def:cqi_protocol} \\
$\mathcal{L}_{\mathrm{all}}$, $\mathcal{L}_{\mathrm{one}}$ & Global (all-copy) loss and one-site marginal loss of a protocol. & \cref{prop:random_purification_cost_functions} \\
$\boldsymbol{p} \dot{=} (p_1, \dots, p_d)$ & Sorted eigenvalue spectrum of a density operator: $p_1 \ge p_2 \ge \dots \ge p_d \ge 0$. & Example~2 (Main Text) \\
$D_{k,i}$ & Spectral gap $p_k - p_i$ between the target $k$-th eigenvalue and the $i$-th eigenvalue. & Example~2 (Main Text) \\
$D_{k,\mathrm{min}}$ & Minimum absolute spectral gap around target eigenvalue $p_k$: $\min_{i \neq k} |p_k - p_i|$. & Example~2 (Main Text) \\
$\yd{\varsigma}$ & Young diagram (YD) indexing the symmetry sectors of the input state under Schur sampling. & Example~2 (Main Text), \cref{subsec:qpa_sample_complexity_supp} \\
$\yt{1\cdots m}$ & Totally symmetric Young tableau of shape $\yd{m}$ representing the fully symmetric output state. & \cref{subsec:eb_povm_supp} \\
$\wt{w}$ & Gel'fand--Tsetlin (GT) basis vector (or semistandard Weyl tableau) specifying a basis state. & \cref{subsec:eb_povm_supp} \\
$\multiset{d}{n}$ & Multiset coefficient $\binom{d+n-1}{n}$, giving the dimension of the symmetric subspace $\mathbb{W}^{\yd{n}}$. & \cref{prop:random_purification_cost_functions} \\
$\extChannel{\mathcal{T}}{\yd{\varsigma}}{\yt{1\dots m}}{\yd{\mu}}$ & Sector-wise covariant QPA channel from input sector $\yd{\varsigma}$ to output $\yt{1\dots m}$ with environment $\yd{\mu}$. & \cref{subsec:eb_povm_supp} \\
$\intertwiner{W}{\yd{\varsigma}}{\yd{\mu}}{\yt{1\dots m}}{}$ & Isometric intertwiner representing the Stinespring dilation of the covariant channel. & \cref{subsec:eb_povm_supp} \\
$\res{f}{\yd{\mu}}{\yd{m}}{\yd{\varsigma}}_{\mathrm{all}}(\wt{w})$ & Restriction coefficient (CGC fidelity component) for a GT basis vector $\wt{w}$. & \cref{subsec:eb_povm_supp}, \cref{eq:constant_eval} \\
$\schur{\yd{\varsigma}}[\boldsymbol{p}]$ & Schur polynomial associated with Young diagram $\yd{\varsigma}$ evaluated on spectrum $\boldsymbol{p}$. & Companion paper, \cref{subsec:optimal_eb_risk_supp} \\
$\weylavg{F}{\boldsymbol{p}}{\yd{\lambda}}$ & Weyl average of function $F$ over semi-standard tableaux of shape $\yd{\lambda}$ weighted by spectrum $\boldsymbol{p}$. & Companion paper \\
$\swavg{X}{\boldsymbol{p}}{m}$ & Schur--Weyl average of sector-wise quantity $X$ under the Schur sampling probability distribution. & \cref{subsec:optimal_eb_risk_supp} \\
$\swprob{\yd{\varsigma}}{d}{m}$ & Schur--Weyl probability mass of symmetry sector $\yd{\varsigma}$ on $m$ copies of state with spectrum $\boldsymbol{p}$. & \cref{subsec:optimal_eb_risk_supp} \\
$\bigO{\cdot}, \bigOm{\cdot}, \bigTheta{\cdot}$ & Asymptotic big-O, big-Omega, and big-Theta notations, respectively. & \cref{sec:risk_symmetry_supp} \\
$\rpoch{a}{k}, \fpoch{a}{k}$ & Rising Pochhammer symbol $(a)^{\overline{k}}$ and falling Pochhammer symbol $(a)^{\underline{k}}$, respectively. & Companion paper \\
\bottomrule
\end{tabularx}
\label{tab:notation}
\caption{Important mathematical notation.}
\end{table}

